Advocate -- Trustworthy Evidence in Cloud Systems

The rapid evolution of cloud-native applications, characterized by dynamic, interconnected services, presents significant challenges for maintaining trustworthy and auditable systems, especially in sensitive contexts, such as finance or healthcare. Traditional methods of verification and certification are often inadequate due to the fast-past and dynamic development practices common in cloud computing. This paper introduces Advocate, a novel agent-based system designed to generate verifiable evidence of cloud-native application operations. By integrating with existing infrastructure tools, such as Kubernetes and distributed tracing systems, Advocate captures, authenticates, and stores evidence trails in a tamper-resistant manner. This approach not only supports the auditing process but also allows for privacy-preserving evidence aggregation. Advocate's extensible architecture facilitates its deployment in diverse environments, enabling the verification and adherence to policies and enhance trust in cloud services.

==> misc/01_introduction.tex <==
% Similar to the motivation in TrustOps/D5.2\

% But we frame it as a tool for generic cloud-native
Cloud-native applications are characterized as highly dynamic, quickly iterating applications that often consist of several interdependent and interconnected services.
These services are often a mixture of managed and self-developed components that together deliver highly scalable, available, and elastic applications using public cloud providers.

Thus, consumers of these applications will have difficulty verifying or understanding how such an application is delivering responses. 
It can be unclear which version of an application was used, in which environment (hardware) this application ran on, and which other cloud services were used. 
While an average consumer may not need this information, it may become critical in sensitive contexts such as finance, insurance or healthcare.
Hence, modern cloud-native applications can quickly clash with the need to provide trustworthy and auditable software. 
Classical approaches, such as formal verification or software process certifications are too time consuming and may not extend to the cloud-providers.

To address this dichotomy, of dynamic fast paced application operation and auditable trustworthy applications, we propose Advocate. 
A new approach that acknowledges the imperfect and changing environment of cloud-native applications while still providing a best effort approach for generating attested evidence to audit and understand a cloud application's behavior.
Advocate follows the TrustOps\cite{trustOps} oriented approach to collect and provide authenticated and actionable records of the operation of an application, giving the consumer a comprehensive picture of an application's behavior.

% The reminder of this paper is organized as follows \dots{}

==> misc/02_advocate.tex <==
%What we need to archive here is to introduce the terminology and benefit. We can also introduce the abstract flow of <events> -> <observation> -> evidence -> claims -> claim aggregations -> claims 
%Advocate -- an \textbf{A}gent for \textbf{D}ata \textbf{V}erification, \textbf{O}n-\textbf{C}haining and \textbf{A}nchoring in \textbf{T}rustless Environments -- is an agent-based system that can be integrated into a cloud-based environment.

%1. Whats a cloud-native system (kubernetes)
Since cloud-native environments are consisting of many different, managed and self-configured services, it is important that our agent can observe and monitor each part of an application that uses this environment.
For example, in case of Kubernetes, 
%one of the most widely used orchestrates for providing cloud-based microservice applications, 
this means that Advocate must have access to the Kubernetes cluster, and be one of the first components to interact with such a cluster when it is deployed. 
%This way, advocate is able to observe changes and events within this cluster to later turn into evidence.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\columnwidth,trim={7 7 7 7},clip]{figures/evidence-in-out}
%     \caption{\todo{A figure caption.}}
%     \label{fige:eidence-in-out}
% \end{figure}

%2. What happens in these systme, why is trust here difficult (lots of moving parts from differnet actors and sotfware componentes0
Operations in such an environment are also characterized by \textit{a mixture of infrastructure and application based actions}. 
% For example, while a developer in for a Kubernetes microservice defines what software 
For example, in a Kubernetes microservice, a developer defines what software to run, Kubernetes (the infrastructure) makes decisions about how many replicas should be deployed, while yet another infrastructure component decides how many virtual machines of what type Kubernetes has access to run this software. 
% Thus, advocate must be able to observe both actions of the application and the actions of the infrastructure, as well as changes to the configuration of both to provide a seamless record of how software was deployed.
Thus, Advocate must be able to observe both actions and changes in the configuration of the application and infrastructure to provide a seamless record of how software was deployed.

% 3. What is out there? Verified deployementes ... 4. What we want to archive do, is evidence of all actions within this scope.
The approach we follow in Advocate is to combine already existing, and emerging approaches to generated \textbf{attested evidence} of the actions that happen in a cloud environment, that can be later verified. 
%Thus, advocate may collect data from the Kubernetes-Audit log, a distributed tracing system, a deployment validator such as kyverno\footnote{https://kyverno.io}, or deeper integration into the container execution engine such as using Confidential Containers\footnote{https://confidentialcontainers.org}. 
The main objective of Advocate is to take all available tools that allow the lightweight observation and validation of execution and generate attested evidence. 
This attested evidence consists of authenticated and signed logs from the different tools that Advocate integrates with.
Advocate ensures the authenticity of this evidence and is responsible of combining and correlating the collected evidence. 
%Hence, it may alter both infrastructure and application configurations to inject identity information into the collected logs.
Moreover, the gathered evidence is always stored in a tamper-resistant and verifiable way, allowing auditors and observers to later follow an evidence trail when reviewing the interactions of a cloud application.

%5. How do we do this. Claims, EvidenceSources, Aggregation 6. How dose this impove trustworthyness? What can be done with this inplace?
Although the tamper-resistant and authenticated evidence trail is already a way for consumers to build trust in an application's operation, the volume and complexity of this evidence together with the sometimes confidential or at least security-relevant information collected, calls for a further step in Advocate. 
In this last step, Advocate enables downstream aggregation of evidence in a verifiable way. %, e.g., using zero knowledge approaches or privacy preserving pipelines.
Here, Advocate manages the orchestration and distribution of the so generated \textbf{aggregated evidence proofs}. 
With this, Advocate offers means to prove adherence to agreements, e.g., using specific versions of a container in a specific region, using specific resources for processing a consumer request, without revealing any internal details that may be included in the raw evidence trail.
This might also enable further actions, e.g., the automatic payment for providing specific data or the automatic settlement of disputes.


==> sections/03_advocate.tex <==
% What we want to archive with advicate, not how we do it. What we consider evidence, aggregation. How we bootstrap and claim things. What additional things can be integrated, and the bigger picture.
\todo{Don't include to much teadal terminalagy, e.g., FDP/sFDP are not needed. We just call them services }
Data lakes\cite{drexl2022position,gorelik2019enterprise,otto_2021_5675897} are a pivotal approach for managing massive amounts of data coming from  diverse sources, e.g., IoT devices, social networks, and business applications. However,  current solutions still suffer from several limitations and challenges. Among them, the single  party ownership — locking valuable data behind organisational silos hindering the creation of  data-driven ecosystems; the lack of proper data governance -- preventing the creation of  trustworthy data flows across organisations and ensuring data sovereignty, a cloud-centric  view — neglecting vast amounts of resources distributed across the cloud computing  continuum (i.e., the resources located at the edge, fog, and cloud), and the lack of energy  awareness -- as current solutions rarely consider sustainability and energy efficiency aspects.  Advocate is among many projects advancing data spaces by evaluating novel solutions to  tackle these limitations and challenges\cite{varepsilonpiiotataurhoopiacuteeta2020european}.

Due to this focus, there is a necessity for an approach to enable trust between data owners and data consumers across  different organizations and across multiple network and device boundaries present in the  compute continuum. Thus, this approach must enable this trustworthiness not only on an identity  level — i.e., ensuring that the data consumer is who they claim to be — but also on a data  level — i.e., ensuring that the data are delivered as agreed and expected. Moreover, it must enable trustworthiness on a process level — i.e., ensuring that the data are processed  as agreed by all parties and on a compliance level — i.e., ensuring that all parties comply with  the applicable laws and regulations. 

Advocate aims to address these challenges first and foremost by providing evidence of every  interaction within the data exchange process. Specifically, we build a trail of evidence that  tracks how identities are obtained, used and communicated, how data are moved, processed  and stored (once they are shared), what processes are used to provide data to consumers and  where these processes are executed and how they are controlled and lastly by collecting  metadata relevant to evaluate compliance. In particular, Advocate enables the creation of trusted, mediationless and verifiable data flows inside a data lake, across federated data lakes and specifically across  stretched data lakes (i.e., deployed in the continuum). Advocate’s architecture is built on top of  the concept of data mesh, expanding it into stretchable and federated data products, and  leveraging many established tools to ensure easy integration of Advocate tools in all  environments.

Claims in Advocate are recorded from different sources in the federated datalakes environment. For each datalake, claims can be issued by the Catalogue, through changes in the Kubernetes cluster, based on the use of ENS accesses or interactions with the data-provider and data-consumer services  based on tracing and monitoring mechanisms in the federation. To monitor the environment comprehensively, Advocate also offers a policy-based validation framework that can be used by the DLO(datalake operator). This integration involves storing policies related to the expected evidence that should be observed for a data-provider service, so that evidence and access can be continuously checked against these expectations, which themselves create evidence claims. In this way, Advocate offers the capability to continuously and comprehensively generate verifiable evidence of interactions between data-provider  and data-consumer services . This capability, to collect and verify evidence and also to aggregate multiple observations into new evidence is used to enhance the trust of data sharing between different datalakes. With each new expansion of the trust plain we are also expanding the plausibility verification of collected evidence.As part of the trustworthy federation mechanisms in federated datalakes environment, the Advocate also plays a crucial role in various core functionalities, including identification, observable interaction, verification, and attestation.In continue we are explaining shortly how Advocate contributes in each of the core functionalities.
 
In the \textit{identification process}, Advocate uses public/private keys to establish the identities of components within federated environment. For \textit{observable interaction}, Advocate ensures that all interactions within federated environment are recorded in immutable storage, making the data tamper-proof and traceable to the source using the components’ unique IDs. This is achieved by storing logs and traces securely as evidenced by Advocate. In the \textit{verification and proving functionality}, Advocate is responsible for collecting claims and storing them in a claim repository. By recording application-level and platform-level claims and signing them with IDs specific to each actor, Advocate ensures that actions within the environment are verifiable later. Also as mentioned before, by recording policies and regulations and validating and verifying if activities in the environment were allied with defined policies in a specific time period, Advocate can improve the proving mechanism. Finally, the Advocate contributes to the \textit{attestation functionalities} by storing data-provider service policies and all related evidence in a transparent, shared infrastructure. This approach provides both consumers and providers with the means to facilitate and verify attestation. Moreover, the policy-based validation framework allows the DLO to define easy to understand claims that consumers and data owners can review when monitoring the data exchange process.

                                                

==> sections/04_architecture.tex <==
% Detailes on how we implemented things, not directly focused on TEADAL. Showcasing, the Demo we've build as an example or some config files.

\todo{We need to reduce remove anything that is very TEADAL, e.g, DLO/ Catalouges ..., specific visions on the nodes. The selling point should be a tool that can collect evidence in a kubernetes enviroment. In the conclusion wen can then link it's use especially in things like federated data lakes.}

Advocate orchestrates the  evidence collection, summarizes it and then publishes it. The DLO(Data Lake Operator) is responsible for starting  Advocate before any data-provider service can be created. A private/public keypair, issued by the DLO, associated with the DLO is used to then create a Datalake ID which is used to sign  any evidence collected on this data lake. Consequently, there will always be exactly one  Advocate instance per data lake in the federated environment. Once established all collected evidence is then  published in an efficient way in the DocumentStore which acts as the Claims Registry, and  permanently stored in the Immutable Storage as a Verifiable Claims.

\subsection{Advocate Architecture}

Advocate's ability to collect, combine, and store evidence from multiple sources makes it a crucial component in the federated dalalakes. By ensuring that all claims are substantiated with telemetry data, Advocate provides a comprehensive view of the datalake's operations. This holistic approach allows for more effective monitoring, auditing, and compliance, helping organizations meet regulatory requirements and maintain trust with consumers of data-provider services. In Kubernetes-level, these claims range from those representing service deployments within that cluster, e.g., data-provider service creation. In Catalogue-level, claims are a report about consumer interactions, e.g., when creating a contract for consuming an service. These claims are stored along with tracing data from observation tools that substantiate them. Observation tools provide tracing logs and metrics, generating Platform-level evidence that Advocate collects, combines, and immutably stores to justify claims. Tracing logs are also used to provide evidence about data exchanges between services. Moreover, we aim to create reliable and trustworthy monitoring sources by enabling mTLS and signed deployment images for all critical infrastructure services.
 
As shown in Figure 1,The architecture of Advocate is designed to handle a diverse range of evidence sources and types, e.g., Jaeger and kubernetes. By supporting various evidence sources from different providers and integrating seamlessly with existing infrastructure of datalakes, Advocate ensures that the integrity of evidences are maintained across all federated environment and datalakes.The use of public and private keys for signing evidence adds an additional layer of authenticity, making it difficult for unauthorised parties to alter or forge claims alongside with using a blockchain for tamper proof record keeping.
 
In a federated environment, where every datalake has its own instance of Advocate running, we need to aggregate all the evidence and verification from different instances across the datalakes. To achieve this, each Advocate instance in each datalake acts as a gateway and provides evidence to other datalakes. This way other advocate instances can discover, verify and enrich observations and combine evidence to build up a comprehensive picture of data exchanges between data-provider and data-consumer services. Moreover, since advocate uses a shared storage (IPFS) and a public (or accessible) blockchain with smart contracts, other third party implementations can interact and use the evidence created by Advocate across the datalakes if needed.

\subsection{Advocate Deployment Options}
 
During Advocate deployment, both the DLO and the federation can configure Advocate in various ways to ensure compatibility with specific requirements for anchoring evidence. For storing evidence securely and enabling transparent sharing via blockchain, Advocate can connect to either a permissioned blockchain or a public one. During the testing phase, the DLO can utilize a local blockchain for testing purposes. The same flexibility applies to IPFS configuration; Advocate can integrate with any type of IPFS (public, private, embedded) that meets the federation's requirements.
 
The DLO and data providers can determine which services within the federation can and should generate claims and designate which parts of the datalake Advocate should monitor simply by labelling these services in the datalake. The frequency of evidence generation and the polling interval for tracing data can be configured in Advocate to optimise cost-efficiency for different levels of auditing requirements.
 
The configurability of Advocate allows it to adapt to varying levels of auditability across different use cases. In a pilot case of evidence-based medicine, where health research institutions utilize data from a private data centre, the sources of evidence are hospitals and research institutions. The frequency of producing evidence is expected to be high to ensure trustworthiness, given the sensitivity and confidentiality of the data. To further enhance confidentiality for medical data, a private blockchain and private IPFS can be utilized. Similar configurations can be applied to industrial use cases, albeit with a lower frequency of evidence production. However, in regional planning, mobility, and smart viticulture pilot cases, the DLOs may prefer to use a public blockchain with a lower evidence frequency, as the shared data is mostly public and involves actors that are in a commercial or governmental relationship.
 
In conclusion, Advocate plays a vital role in ensuring the trustworthiness and integrity of evidence in datalakes in the federated environment ecosystem. Its ability to integrate, store, and secure evidence from multiple sources, combined with its use of blockchain technology, makes it an indispensable tool for managing and verifying claims. By offering a comprehensive and tamper-proof solution, Advocate helps organizations to share their data products with their stakeholders and build trust with them.

